DASpeech: Directed Acyclic Transformer for Fast and High-quality Speech-to-Speech Translation

Direct speech-to-speech translation (S2ST) translates speech from one language into another using a single model. However, due to the presence of linguistic and acoustic diversity, the target speech follows a complex multimodal distribution, posing challenges to achieving both high-quality translations and fast decoding speeds for S2ST models. In this paper, we propose DASpeech, a non-autoregressive direct S2ST model which realizes both fast and high-quality S2ST. To better capture the complex distribution of the target speech, DASpeech adopts the two-pass architecture to decompose the generation process into two steps, where a linguistic decoder first generates the target text, and an acoustic decoder then generates the target speech based on the hidden states of the linguistic decoder. Specifically, we use the decoder of DA-Transformer as the linguistic decoder, and use FastSpeech 2 as the acoustic decoder. DA-Transformer models translations with a directed acyclic graph (DAG). To consider all potential paths in the DAG during training, we calculate the expected hidden states for each target token via dynamic programming, and feed them into the acoustic decoder to predict the target mel-spectrogram. During inference, we select the most probable path and take hidden states on that path as input to the acoustic decoder. Experiments on the CVSS Fr-En benchmark demonstrate that DASpeech can achieve comparable or even better performance than the state-of-the-art S2ST model Translatotron 2, while preserving up to 18.53x speedup compared to the autoregressive baseline. Compared with the previous non-autoregressive S2ST model, DASpeech does not rely on knowledge distillation and iterative decoding, achieving significant improvements in both translation quality and decoding speed. Furthermore, DASpeech shows the ability to preserve the speaker's voice of the source speech during translation.

==> Sections/210_speech_to_speech.tex <==
Direct speech-to-speech translation (S2ST) aims to convert speech from one language into another in an end-to-end paradigm. Given a source speech, the S2ST model generates the mel-spectrogram \citep{translatotron} or discrete units\footnote{Discrete units are usually derived from a self-supervised speech pretrained model.} \citep{s2ut} corresponding to the target speech, which can be converted into waveform with an additional vocoder. To ease the difficulty of learning complex mappings between speech in different languages, recent works \citep{translatotron2, inaguma2022unity} propose the two-pass architecture, which first generates the target text and then generates the target mel-spectrogram or discrete units based on the representations of the target text, which achieves state-of-the-art translation quality among S2ST models.

==> Sections/430_speedup.tex <==

The speedup ratio in Tables \ref{tab:main} and \ref{tab:multilingual} are evaluated with a batch size of 1. As \citet{gu-kong-2021-fully} pointed out, the speed benefits of non-autoregressive models may degrade during batch decoding. To better understand this problem, we evaluate the speedup ratio under different decoding batch sizes. As shown in Figure \ref{fig:speedup}, the speedup ratio keeps dropping as the decoding batch size increases. Nevertheless, DASpeech ($\lambda=0.5$ with Joint-Viterbi decoding) still achieves more than 6$\times$ speedup with a decoding batch size of 64 and maintains comparable performance with Translatotron 2.



==> Tables/table_best_expect_path.tex <==
\begin{table}[t]
% \begin{wraptable}{r}{0.6\linewidth}
\centering
\small
\caption{ASR-BLEU scores on CVSS-C Fr-En \texttt{test} set with best-path training and expect-path training.}
% \resizebox{\linewidth}{!}{
\begin{tabular}{ll|cc|c}
\toprule
\textbf{Models} & & \textbf{Best} & \textbf{Expect} & \textbf{\Delta} \\
\midrule
\multicolumn{1}{c|}{\textbf{DASpeech}} & + Lookahead   & 24.47 & 24.70 & +0.23 \\
\multicolumn{1}{c|}{($\lambda=0.5$)} & + Joint-Viterbi & 24.73 & 25.04 & +0.31 \\
\midrule
\multicolumn{1}{c|}{\textbf{DASpeech}} & + Lookahead   & 24.22 & 24.42 & +0.20 \\
\multicolumn{1}{c|}{($\lambda=1.0$)} & + Joint-Viterbi & 24.44 & 24.79 & +0.35 \\
\bottomrule
\end{tabular}
% }
\label{tab:path_ablation}
\end{table}
% \end{wraptable}

==> Tables/table_multilingual.tex <==
\begin{table}[t]
% \begin{wraptable}{r}{0.6\linewidth}
\centering
\small
\caption{Results on CVSS-C \texttt{test} sets of the multilingual X$\rightarrow$En S2ST model. The detailed results can be found in the supplementary material.}
% \resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccc|c}
\toprule
\multirow{2}{*}{\textbf{Models}} & & \multicolumn{4}{c|}{\textbf{ASR-BLEU (X$\rightarrow$En)}} & \multirow{2}{*}{\textbf{Speedup}} \\
 & & \textbf{Avg.} & \textbf{High} & \textbf{Mid} & \textbf{Low} & \\
\midrule
\multicolumn{2}{l|}{Translatotron 2 \citep{translatotron2}} & \textbf{8.73} & \textbf{25.96} & \textbf{11.06} & \textbf{2.03} & 1.00$\times$ \\
\multicolumn{2}{l|}{UnitY \citep{inaguma2022unity}} & 8.15 & 24.97 & 9.78 & 1.86 & 1.01$\times$ \\
\midrule
\multicolumn{1}{c|}{\textbf{DASpeech}} & + Lookahead & 7.22 & 22.70 & 8.63 & 1.48 & \textbf{12.96$\times$} \\
\multicolumn{1}{c|}{($\lambda=1.0$)} & + Joint-Viterbi & 7.21 & 22.55 & 8.68 & 1.48 & 10.99$\times$ \\
\bottomrule
\end{tabular}
% }
\label{tab:multilingual}
\end{table}
% \end{wraptable}
